A Discriminative Single-Shot Segmentation Network for Visual Object Tracking

Template-based discriminative trackers are currently the dominant tracking paradigm due to their robustness, but are restricted to bounding box tracking and a limited range of transformation models, which reduces their localization accuracy. We propose a discriminative single-shot segmentation tracker -- D3S2, which narrows the gap between visual object tracking and video object segmentation. A single-shot network applies two target models with complementary geometric properties, one invariant to a broad range of transformations, including non-rigid deformations, the other assuming a rigid object to simultaneously achieve robust online target segmentation. The overall tracking reliability is further increased by decoupling the object and feature scale estimation. Without per-dataset finetuning, and trained only for segmentation as the primary output, D3S2 outperforms all published trackers on the recent short-term tracking benchmark VOT2020 and performs very close to the state-of-the-art trackers on the GOT-10k, TrackingNet, OTB100 and LaSoT. D3S2 outperforms the leading segmentation tracker SiamMask on video object segmentation benchmarks and performs on par with top video object segmentation algorithms.

==> cutout.tex <==
D3S estimates target size with the TSM during tracking by combining segmentation mask predicted by the refinement pathway and backbone template~($\mathbf{X}_0$) and search features~($\mathbf{X}_t$). 
An overall architecture of the TSM is shown in Figure~\ref{fig:scale-change-module-scheme}. 

Since the predicted mask is in image coordinates, which is 16-times larger than resolution of the features, we reduce the mask resolution using mask downsampling module (MDM), shown in Figure~\ref{fig:mask-downsampling}. 
Furthermore, a $1\times 1$ convolution is used to reduce the number of channels in $\mathbf{X}_0$ and $\mathbf{X}_t$. 
The reduced features and downsampled mask are combined using the classification and target region heads. 
Both heads have the same architecture, shown in Figure~\ref{fig:head-architecture}. 

{\bf Target classification head} (TCH) 
predicts two channels, which represent target and background presence scores. 
Position of the maximum in the per-pixel softmax between these two channels represents the most likely target position, denoted as $\tilde{\mathbf{p}}$. 

{\bf Target region head} (TRH) 
predicts four channels $\mathbf{d}_{\mathrm{T}}$, $\mathbf{d}_{\mathrm{B}}$, $\mathbf{d}_{\mathrm{R}}$ and $\mathbf{d}_{\mathrm{L}}$, 
where value on each element is a distance from this element to the top, bottom, right and left edges of the target bounding box, respectively. 
Target width ($\tilde{w}$) and height ($\tilde{h}$) are calculated as
\begin{equation} 
    \tilde{w} = \mathbf{d}_{\mathrm{R}}(\tilde{\mathbf{p}}) - \mathbf{d}_{\mathrm{L}}(\tilde{\mathbf{p}}),
\end{equation}
\begin{equation} 
    \tilde{h} = \mathbf{d}_{\mathrm{T}}(\tilde{\mathbf{p}}) - \mathbf{d}_{\mathrm{B}}(\tilde{\mathbf{p}}),
\end{equation}
where $\mathbf{d}_{\mathrm{( \cdot )}}(\tilde{\mathbf{p}})$ denotes the value on the one position $\tilde{\mathbf{p}}$ in one of the four TRH channels.
--------------------------------------------------------------------------------
